The International Large Detector: Letter of Intent

The International Large Detector (ILD) is a concept for a detector at the International Linear Collider, ILC. The ILC will collide electrons and positrons at energies of initially 500 GeV, upgradeable to 1 TeV. The ILC has an ambitious physics program, which will extend and complement that of the Large Hadron Collider (LHC). A hallmark of physics at the ILC is precision. The clean initial state and the comparatively benign environment of a lepton collider are ideally suited to high precision measurements. To take full advantage of the physics potential of ILC places great demands on the detector performance. The design of ILD is driven by these requirements. Excellent calorimetry and tracking are combined to obtain the best possible overall event reconstruction, including the capability to reconstruct individual particles within jets for particle ow calorimetry. This requires excellent spatial resolution for all detector systems. A highly granular calorimeter system is combined with a central tracker which stresses redundancy and efficiency. In addition, efficient reconstruction of secondary vertices and excellent momentum resolution for charged particles are essential for an ILC detector. The interaction region of the ILC is designed to host two detectors, which can be moved into the beam position with a push-pull scheme. The mechanical design of ILD and the overall integration of subdetectors takes these operational conditions into account.

==> authors/ILDorganisation.tex <==
\begin{flushright}
\section*{ILD Organisation}
\end{flushright}

\noindent The following table lists the names of the members of the ILD organisation as of March 2009. \hfill

\vspace{5mm}
%\begin{center}
\begin{tabular}{ll}
{\bf Joint Steering Board} & 
%\begin{minipage}[l]{8cm}
Ties Behnke,
Dean Karlen,
Yasuhiro Sugimoto,\\
& Henri Videau,
Graham Wilson,
Hitoshi Yamamoto\\
%\end{minipage} \\
{\bf ILD Working Groups} & \\
Detector optimisation & 
%\begin{minipage}[l]{8cm}
Mark Thomson,
Yosuke Takubo\\
%\end{minipage}\\
Integration/ Machine Detector Interface & 
%\begin{minipage}[l]{8cm}
Karsten B\"usser,
Toshiaki Tauchi\\
%\end{minipage}\\
Costing & 
%\begin{minipage}[l]{8cm}
Tomoyuki Sanuki,
Henri Videau\\
%\end{minipage}\\
Software and Tools& 
Frank Gaede,
Akiya Miyamoto\\
{\bf Subdetector Contacts} & \\
Vertex & 
%\begin{minipage}[l]{8cm}
Marc Winter,
Yasuhiro Sugimoto\\
%\end{minipage}\\
Silicon tracking & 
%\begin{minipage}[l]{8cm}
Aurore Savoy-Navarro,
Hwanbae Park\\
%\end{minipage}\\
TPC & 
%\begin{minipage}[l]{8cm}
Ron Settles,
Keisuke Fujii\\
%\end{minipage}\\
ECAL & 
%\begin{minipage}[c]{8cm}
Jean Claude Brient,
Kiyotomo Kawagoe\\
%\end{minipage}\\
HCAL & 
%\begin{minipage}[c]{8cm}
Imad Laktineh,
Felix Sefkow\\
%\end{minipage}\\
FCAL& 
%\begin{minipage}[c]{8cm}
Wolfgang Lohmann\\
%\end{minipage}\\
Muon & 
%\begin{minipage}[c]{8cm}
Vishnu Zutshi\\
%\end{minipage}\\
Data Acquisition & 
%\begin{minipage}[c]{8cm}
G\"unter Eckerlin\\
%\end{minipage}
Coil & 
Francois Kircher\\
\end{tabular}

%\end{center}

==> optimization/fsimulation.tex <==
\section{Tools for Performance Studies}

The optimisation of the ILD concept was performed in parallel using 
the software tools developed by the GLD and the LDC detector concept 
groups.  For this study six detector models were defined; 
three based on the GLD detector simulation (GLD, GLDPrime and GLD4LDC) 
and three based on the LDC detector simulation (LDC, LDCPrime, 
and LDC4GLD). The detector simulation was performed using GEANT4 
(version 9.1 patch01) with the {\tt LCPhysicsList} physics list. 
The main parameters of the models are summarised in 
Table~\ref{tab:optdetparameter}. The models 
represent different compromises between magnetic 
field and TPC outer radius: B = 4.0\,T and $R_{max} \approx 1.5$\,m 
(LDC and GLD4LDC);  B = 3.5\,T and $R_{max} \approx 1.75$\,m
(GLDPrime and LDCPrime); and  B = 3.0\,T and $R_{max} \approx 1.95$\,m
(GLD and LDC4GLD). The software frameworks (JSF and Mokka/Marlin) used to simulate and reconstruct
the detector models are summarised below. 

\begin{table}
\begin{center}
\caption{Parameters of baseline detector models used for the optimisation studies
         (GLD, GLDPrime, GLD4LDC, LDC4GLD, LDCPrime and LDC). Also shown are
     the corresponding parameters for the ILD baseline detector.  
     Unless otherwise specified, values are shown in the units of mm.
\label{tab:optdetparameter}}
{\tabcolsep=0.07cm
\begin{tabular}{|l|l||c|c|c|c|c|c||c|} \hline
\multicolumn{2}{|l||}{Model Name} 
& GLD & GLD$^\prime$ & GLD4LDC & LDC4GLD & LDC$^\prime$ & LDC & ILD \\ \hline
\multicolumn{2}{|l||}{Simulator}
& \multicolumn{3}{|c| }{Jupiter} & \multicolumn{3}{|c||}{Mokka} & Mokka \\ \hline
\multicolumn{2}{|l||}{B field (T)} 
&  3.0 & 3.5 & 4.0 & 3.0 & 3.5 & 4.0 & 3.5 \\ \hline
\multicolumn{2}{|l||}{Beampipe R$_{min}$}
 & 15.0 & 14.0 & 13.0 & 15.5 & 14.0 & 13.0 & 14.5 \\ \hline
Vertex & 
 Geometry & \multicolumn{3}{|c|}{cylindrical} & \multicolumn{3}{|c||}{ladders}
 & ladders \\ \cline{2-9}
 Detector & Layers & \multicolumn{3}{|c|}{3 doublets} & \multicolumn{3}{|c||}{5}
 &3 doublets\\ \cline{2-9}
 &
R$_{min}$& 17.5 & 16.0 & 15.0 & 16.5 & 15.0 & 14.0 & 16.0 \\ \hline
%~~~Thickness & \multicolumn{6}{|c|}{0.1\% rad. len. / layers } \\ \hline 
Barrel&
Layers & \multicolumn{3}{|c|}{4 cylinders} & \multicolumn{3}{|c||}{2 cylinders} & 2 cylinders\\ \cline{2-9}
SIT & Radii & \multicolumn{3}{|c|}{90, 160, 230, 300} & \multicolumn{3}{|c||}{161.4, 270.1} & 165, 309\\ \hline
%~~~Thickness & \multicolumn{3}{|c|}{0.6\% rad. len. / layers} & \multicolumn{3}{|c|}{0.7\% rad. len / layers } \\ \hline
TPC & R$_{min}$ &  437 &  435 &  371 & \multicolumn{3}{ |c|| } {371 } & 395 \\ \cline{2-9}
drift & R$_{max}$ & 1978 & 1740 & 1520 & 1931 & 1733 & 1511 & 1739 \\ \cline{2-9} 
region &  $z_{max}$ & ~~2600~~ & ~~2350~~ & ~~2160~~ & ~~2498~~ & ~~2248~~ & ~~2186~~ & ~~2247.5~~ \\ \hline
\multicolumn{2}{|l||}{TPC pad rows} & 256 & 217 & 196 & 260 & 227 & 190 & 224 \\ \hline
ECAL & R$_{min}$ & 2100 & 1850 & 1600 & 2020 & 1825 & 1610 & 1847.4\\ \cline{2-9}
barrel & Layers & \multicolumn{3}{|c|}{33} &  \multicolumn{3}{|c||}{20(thin)+9(thick)} & 20+9\\ \cline{2-9}
 & Total $X_0$ & \multicolumn{3}{|c|}{28.4} &  \multicolumn{3}{|c||}{22.9} & 23.6 \\ \hline
\multicolumn{2}{|c||}{ECAL endcap z$_{min}$} & 2800 & 2250 & 2100 &  2700 & 2300 & 2550 & 2450 \\ \hline
HCAL & Layers & 46 & 42 & 37  & \multicolumn{3}{|c||}{48} & 48 \\ \cline{2-9}
barrel  & R$_{max}$ & 3617 & 3260 & 2857 & 3554 & 3359 & 3144 & 3330 \\ \hline
\multicolumn{2}{|l||}{Total $\lambda_I$} & 6.79 & 6.29 & 5.67 &  \multicolumn{3}{|c||}{6.86} & 6.86 \\ \hline 
\end{tabular}
}
\end{center}
\end{table}
%%}


\subsection{GLD Software: JSF}

JSF\cite{ref:jsf} is a root based software framework for modular applications, 
such as event generation, fast and full simulation, 
event reconstruction and data analysis. The two main components are
Jupiter\cite{ref:jupiter} and Satellites\cite{ref:satellites}.
Jupiter is a GEANT4\cite{ref:geant4} based detector
simulation, designed to enable easy installation/modification of sub-detector 
components. Satellites\cite{ref:satellites} is a collection of event 
reconstruction modules in the JSF framework. Satellites includes 
smearing of hit points simulated by Jupiter, a ``cheated'' track finder
using Monte Carlo information to associated hits to tracks, 
a Kalman filter-based track fitter, and a cheated particle flow algorithm (PFA).

Jupiter reads a set of detector parameters at run time from a text file,
which makes it easy to study different detector configuration.
The geometry information is saved in a output root file for use by event reconstruction,
when executed as a JSF application. 
%A typical detector geometry of Jupiter is shown in 
%\ref{fig:Tools-GLDGeometry}.
%\begin{figure}
%\begin{center}
%\includegraphics[width=7cm]{gldmar08-2div-mod.eps}
%\label{fig:tools-GLDGeometry}
%\caption{GLD geometry in Jupiter}
%\end{center}
%\end{figure}
A typical Jupiter model consists of beam pipes, vertex detectors (VTX), 
intermediate silicon trackers (IT), a
TPC, endcap and barrel calorimeters, solenoid magnets, muon detectors,
forward electromagnetic calorimeters, a low angle ``beam'' calorimeter,
and support structures.  The vertex detector and intermediate silicon trackers 
are modelled as cylinders.  The calorimeters have a 12-fold symmetry.
The electromagnetic calorimeter consists of layers consisting of 
3\,mm tungsten absorber, 2\,mm scintillator sensor, and a 1\,mm air gap.
The hadron calorimeter consists of layers of an iron absorber, a 
scintillator sensor, and air gap with thickness 20\,mm, 5\,mm and 1\,mm, 
respectively. The scintillator in both the ECAL and HCAL is segmented into
1x1\,cm$^{2}$ readout tiles. Signals in each tiles are summed up at the time 
of reconstruction to simulate the strip shape readout structure of proposed system.
In the version of the simulation used for the studies there was no gap 
between the ECAL and HCAL. 

Jupiter was executed as a module of JSF and exact hits information of each 
sensitive detector were
saved as a root file for subsequent study by Satellites package or as an LCIO 
file for reconstruction by MarlinReco packages.  

The point resolution of the tracking chambers was implemented in the 
Satellites reconstruction. The exact GEANT 4 hit points in the VTX 
and IT were smeared with a Gaussian with fixed resolutions. For the
VTX  $\sigma_{r\phi}$ and $\sigma_{z}$ where set to 2.8$\mu$m. 
For barrel silicon tracker, a resolution of 10\,$\mu$m was used for 
both $\sigma_{r\phi}$ and $\sigma_{z}$.
%, while studies by Mokka used 4 $\mu m$ for $\sigma_{r\phi}$ and
%50 $\mu m$ for $\sigma_{Z}$.
The TPC space points were smeared by Gaussian resolutions, $\sigma_{r\phi}$ and $\sigma_{z}$,
given by following equations:
\begin{eqnarray*}
\sigma^2_{r\phi}&=&50^2+900^2\sin^2\phi + \left( (25^2/22)\times (4/B)^2\sin\theta\right) z \,\mu\mathrm{m}^2;\\
\sigma^2_{z}&=&40^2+8^2\times z \,\mu\mathrm{m}^2;
\end{eqnarray*}
where $z$ is the drift length in cm,  $B$ is the magnetic field strength 
in Tesla, and $\theta$  and $\phi$ are the track angles with 
respect to the line perpendicular to the pad plane and the one to the pad rows.
For the calorimeter, no additional smearing is applied at reconstruction time;
the simulated energy deposits in the scintillator tiles are used directly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- Description of Marlin, Mokka, MarlinReco, PandoraPFA, LCFIVertex, Tracking, ...
\subsection{LDC Software: Mokka and Marlin}

The software framework developed by the LDC concept is based on the LCIO \cite{ref:lcio}
persistency format and event data model. The detailed simulation of the 
detector response is performed by the GEANT4\cite{ref:geant4} based
Mokka\cite{ref:mokka} application.  The sub-detector geometries and materials
used in the structures are stored in a MySQL database. The overall detector
is then built from individual sub-detectors, making it relatively straightforward 
to compare different technology choices. 
The corresponding {\tt C++} code instantiating the sub-detector geometry in memory
is written such that the whole detector model can be scaled in length and radius; this
feature proved invaluable in optimising the detector geometry.
The Gear\cite{ref_gear} tool provides access to these geometrical detector properties 
at the reconstruction and analysis level, where {\tt XML} files are used to store the main
detector parameters. 

The Mokka generated events are processed in Marlin\cite{ref_marlinlccd}. Marlin is a 
modular {\tt C++} application framework which supports plugin modules (called processors)
which can be loaded at runtime, with the modules specified in an {\tt XML} 
configuration file. This plugin-based design supports the distributed 
development of reconstruction algorithms and also allows comparison of
different algorithms runtime, {\it e.g.} it is possible to run two
tracking algorithms producing parallel collections of reconstructed
tracks.

Event reconstruction is performed with the MarlinReco package. This consists of a set of
Marlin reconstruction modules for digitisation, track finding, track fitting, 
particle flow reconstruction, and flavour tagging.
The hit smearing for the tracking detectors is implemented at the digitisation stage using the
same parameterisation as used for Satellites, except that resolutions for the
intermediate silicon tracker (SIT) are taken to be 4\,$\mu$m for $\sigma_{r\phi}$ and 
50\,$\mu$m for $\sigma_{z}$. The pattern recognition processors use Kalman Filter techniques 
and code developed for the LEP experiments. Tracks from standalone pattern recognition in the 
silicon trackers and in the TPC are combined and refitted, providing extremely good momentum 
resolution (see section \ref{sec:trackperform}).
Reconstruction of the individual particles in the event is done with the particle flow algorithm
in the PandoraPFA \cite{ref:pandorapfa} package that provides the currently best such algorithm.
The LCFIVertex \cite{ref:lcfivertx} package provides code for vertex finding and 
fitting and the identification of short
lived heavy particles using a neural network approach as well as jet charge estimation.
Some further analysis algorithms for jet finding and kinematic fitting are available in MarlinReco.
%%The core framework is completed by the LCCD\cite{ref_marlinlccd} conditions
%%data toolkit mainly used in R\&D testbeam studies.


\subsection{GLD and LDC Detector Optimisation Studies}

The studies in the LDC framework are based on full reconstruction
of the simulated events; at no stage is Monte Carlo information
used. The studies in the GLD framework use the Satellites reconstruction
and PandoraPFA for particle flow reconstruction. The interoperability 
between the two software frameworks is provided by the LCIO data format, 
{\it e.g.} after simulating the detector response with the Jupiter program, 
MarlinReco and PandoraPFA were used for the event reconstruction.
The same generated events ({\tt STDHEP} files) where simulated in
the models listed in Table~\ref{tab:optdetparameter}. In addition,
variations on the LDCPrime model where used to study particle flow 
performance.

% \end{tiny}




==> optimization/optimization.tex <==
%optimization chapter
\writer{Mark Thomson, Yoshioka Tamaki}

==> optimization/performance-tool.tex <==
\section{Tools for Performance Studies}
%\writer{Akiya Miyamoto and Frank Gaede}

%\newcommand{\fixme}[1]{\textsf{\textbf{(#1)}}} % command for comments 

ILD has been optimized by using software tools developed by GLD and LDC group.

Tools developed by GLD group consists of JSF, Jupiter, Satellites, and 
other utility tools.
JSF\cite{ref:jsf} is a root based framework for modular applications, such as event generation, 
fast and full simulation, reconstruction and test data analysis. Jupiter\cite{ref:jupiter} is a Geant4\cite{ref:geant4} simulator
designed with an emphasis of easy installation/un-installation of sub-detector 
components. Satellite\cite{ref:satellites} is a collection of JSF module for event reconstruction. 
Functions of Satellites includes 
smearing of exact hit points simulated by Jupiter, cheated track finder,
track fitting by Kalman fitter, and cheated PFA, first three of them being 
used for the performance studies described in the next section.  

Jupiter reads a set of detector parameters at run time from a text file,
which makes it easy to study different detector configuration.
The geometry information is saved in a output root file for use by event reconstruction,
when executed as a JSF application. 
%A typical detector geometry of Jupiter is shown in 
%\ref{fig:Tools-GLDGeometry}.
%\begin{figure}
%\begin{center}
%\includegraphics[width=7cm]{gldmar08-2div-mod.eps}
%\label{fig:tools-GLDGeometry}
%\caption{GLD geometry in Jupiter}
%\end{center}
%\end{figure}
A typical Jupiter model consists of beam pipes, vertex detectors (VTX), inter-mediate silicon trackers(IT),
TPC, endcap and barrel calorimeters, solenoid magnets, muon detectors,
forward elemag calorimeter, beam calorimeter,
and other support materials.  Vertex detector and inter-mediate silicon trackers 
are approximated by cylinder.  Calorimeter has a 12-folded shape, with a read out tile size of 
1x1 cm$^{2}$. Signals in each tiles are summed up at the time of reconstruction to 
simulate a strip shape readout structure of proposed system.
Each layer of electromagnetic calorimeter section consists of tungsten absorber, scintillator sensor,
and gap of air, with thickness being 3~mm, 2~mm, and 1~mm respectively.  
Layers of hadron calorimeter consists of iron absorber, scintillator sensor, 
and gap of air with thickness 20~mm, 5~mm and 1~mm, respectively. 
No gap between calorimeter structure were defined.
Jupiter was executed as a module of JSF and exact hits information of each sensitive detector were
saved as a root file for subsequent study by Satellite package or as an LCIO 
file for reconstruction by MarlinReco packages.  

When smearing detector signals in Sattelites, exact hit points in VTX 
and IT were gaussian-smeared with a fixed resolution. $\sigma_{r\phi}$ and 
$\sigma_{Z}$ of VTX was 2.8$\mu m$. For barrel silicon tracker,
studies by Jupiter used 10 $\mu m$ for both $\sigma_{r\phi}$ and
$\sigma_{Z}$.
%, while studies by Mokka used 4 $\mu m$ for $\sigma_{r\phi}$ and
%50 $\mu m$ for $\sigma_{Z}$.
On the other hand, 
the TPC space points are gaussian-smeared by resolutions, $\sigma_{r\phi}$ and $\sigma_{Z}$,
whose resolution in the unit of $\mu m$ is given by following equations:
\begin{eqnarray}
\sigma^2_{r\phi}&=&50^2+900^2\sin^2\phi + \left( (25^2/22)\times (4/B)^2\sin\theta\right) L\\
\sigma^2_{Z}&=&40^2+8^2\times L
\end{eqnarray}
where $L$ is the drift length in unit of cm and $B$ is the field strength 
of the solenoid magnet in unit of Tesla. $\theta$  and $\phi$ is the track angle with 
respect to the line perpendicular to the pad plane and the one to the pad rows.
Concerning the calorimeter, energy deposits to the sensitive detector 
are used as its signal.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- Description of Marlin, Mokka, MarlinReco, PandoraPFA, LCFIVertex, Tracking, ...
The software framework developed by the LDC concept is fully based on the LCIO \cite{ref:lcio}
persistency format and event data model that is also used by other detector concepts in the
ILC community. The detailed simulation of the detector response is done in the geant4\cite{ref:geant4} based
Mokka\cite{ref:mokka} application.  The geometrical and material parameters of the detector
are stored in a MySQL database on a per subdetector basis making it easy to compare different
technology choices. The corresponding C++ code instantiating the subdetector geometry in memory
is written such that the whole detector model can be scaled in length and radius - a feature that 
proved very useful in optimsing the detector geometry.
The Gear\cite{ref_gear} tool provides access to these geometrical detector properties at the reconstruction
and analaysis level, where xml files are used to transfer the needed paremeters.
This further processing is done in Marlin\cite{ref_marlinlccd},  a modular C++ application framework.
The modules - called processors - are implemented as plugin components that can be loaded at runtime
as specified in the xml configuration file. This plugin based design supports the distributed 
development of reconstruction algorithms and allows to freely exchange these
algorithms for cross comparisons at runtime.

MarlinReco is a package of Marlin modules for reconstruction, in particular for digitisation
and tracking. 
%Some processors performe a rather detailed simulation 
%of the readout electronics while others apply a parameterised digitisation of the
%simulated hits. The latter strategy is used for the optimisation and performance studies presented 
%in this document, where the parameterisation is based on the latest R&D results 
%for the various subdetectors.
The same parameterized digitization as the one described above for the Satellites tool is applied, except that
4 $\mu m$ for $\sigma_{r\phi}$ and 50 $\mu m$ for $\sigma_{Z}$ in the intermeditate silicon tracker are used.

The pattern recognition processors use Kalman Filter techniques and code developed for the LEP
experiments. Tracks from standalone pattern recognition in the silicon trackers and in the TPC are combined and 
refitted, providing extremely good momentum resolution (see section \ref{sec:trackperform}).
Reconstruction of the individual particles in the event is done with the particle flow algorithm
in the PandoraPFA \cite{PandoraPFA} package that provides the currently best such algorithm.
The LCFIVertex \cite{ref:lcfivertx} package provides code for vertex finding and fitting and the identification of short
lived heavy particles using a neural network approach as well as jet charge estimation.
Some further analysis algorithms for jet finding and kinematical fitting are available in MarlinReco.

LCIO provides the basis for interoperability between the two frameworks, as
data files can be exchanged at the various levels of the data processing, e.g. after simulating 
the detector response with the Jupiter program, MarlinReco and PandoraPFA can be used for 
event reconstruction.
The core framework is completed by the LCCD\cite{ref_marlinlccd} conditions
data toolkit mainly used in R\&D testbeam studies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to study detector performances six detector models were defined. 
Major parameter of them
are summarized in the table \ref{tab:optdetparameter}.  GLD, GLD'
and J4LDC were defined for Jupiter and LDC, LDCPrime, and LDC-GLD 
were defined for Mokka.  J4LDC has similar dimension as LDC, 
LDC-GLD is similar to GLD, and GLD' and LDC' is 
intermediate size of GLD and LDC.
The version number of Geant4 used for the optimization was 
9.1 patch01 and the physics list was LCPhysicsList. 


\begin{table}
\caption{Parameters of detector models for optimization.  Values are shown in the unit of mm,
unless otherwise specified.}
\label{tab:optdetparameter}
\begin{center}
%\begin{tiny}
{\tabcolsep=0.07cm
\begin{tabular}{|l|l||c|c|c|c|c|c||c|} \hline
\multicolumn{2}{|l||}{Model Name} 
& GLD & GLD' & J4LDC & LDC-GLD & LDC' & LDC & ILD\_00 \\ \hline
\multicolumn{2}{|l||}{Simulator}
& \multicolumn{3}{|c| }{Jupiter} & \multicolumn{3}{|c||}{Mokka} & Mokka \\ \hline
\multicolumn{2}{|l||}{B field (T)} 
&  3 & 3.5 & 4 & 3 & 3.5 & 4 & 3.5 \\ \hline
\multicolumn{2}{|l||}{Beam pipe R$_{min}$}
 & 15 & 14 & 13 & 15.5 & 14 & 13 & 14.5 \\ \hline
Vertex & 
 Structure & \multicolumn{3}{|c|}{Cylindrical, 3 double layers} & \multicolumn{3}{|c||}{5 layers ladder}
 & 3 double laders\\ \cline{2-9}
Detector &
R$_{min}$& 17.5 & 16 & 15 & 16.5 & 15 & 14 & 16 \\ \hline
%~~~Thickness & \multicolumn{6}{|c|}{0.1\% rad. len. / layers } \\ \hline 
Barrel&
No. layers & \multicolumn{3}{|c|}{4 cylinders} & \multicolumn{3}{|c||}{2 cylinders} & 2 cylinders\\ \cline{2-9}
SIT & R$_{min}$ & \multicolumn{3}{|c|}{90, 160, 230, 300} & \multicolumn{3}{|c||}{161.4, 270.1} & 165, 309\\ \hline
%~~~Thickness & \multicolumn{3}{|c|}{0.6\% rad. len. / layers} & \multicolumn{3}{|c|}{0.7\% rad. len / layers } \\ \hline
TPC & R$_{min}$ &  437 &  435 &  371 & \multicolumn{3}{ |c|| } {371 } & 395 \\ \cline{2-9}
drift & R$_{max}$ & 1978 & 1740 & 1520 & 1931 & 1733 & 1511 & 1739 \\ \cline{2-9} 
region & Half Z length & ~~2600~~ & ~~2350~~ & ~~2160~~ & ~~2498~~ & ~~2248~~ & ~~2186~~ & ~~2247.5~~ \\ \hline
\multicolumn{2}{|l||}{TPC No. of pad rows} & 256 & 217 & 196 & 260 & 227 & 190 & 224 \\ \hline
ECAL & R$_{min}$ & 2100 & 1850 & 1600 & 2020 & 1825 & 1610 & 1847.4\\ \cline{2-9}
barrel & No. layers & \multicolumn{3}{|c|}{33} &  \multicolumn{3}{|c||}{20(thin)+9(thick)} & 20+9\\ \cline{2-9}
 & Rad. len. ($X_0$) & \multicolumn{3}{|c|}{28.4} &  \multicolumn{3}{|c||}{22.9} & 23.6 \\ \hline
\multicolumn{2}{|c||}{ECAL Endcap Z$_{min}$} & 2800 & 2250 & 2100 &  2700 & 2300 & 2550 & 2450 \\ \hline
HCAL & No. layers & 46 & 42 & 37  & \multicolumn{3}{|c||}{48} & 48 \\ \cline{2-9}
barrel  & R$_{max}$ & 3617 & 3260 & 2857 & 3554 & 3359 & 3144 & 3330 \\ \hline
\multicolumn{2}{|l||}{Total Int. length ($\lambda$)} & 6.79 & 6.29 & 5.67 &  \multicolumn{3}{|c||}{6.86} & 6.86 \\ \hline
\end{tabular}
}

% \end{tiny}
\end{center}
\end{table}




==> performance/physics_gmsb.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\subsection{$\tilde{\chi^0_1}\tilde{\chi^0_1} \to \gamma \tilde{G} \gamma \tilde{G}$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this Gauge-Mediated SUSY Breaking (GMSB) scenario, the
next-to-lightest SUSY particle (a neutralino $\tilde{\chi}^0_1$) will
inevitably decay into the lightest SUSY particle (a Gravitino
$\tilde{G}$) and its SM partner (a photon $\gamma$). As defined
in~\cite{benchmark-note}, the neutralino mass is $151.1~\rm{GeV}$. For
a life\-time of $\tau_{\tilde{\chi^0_1}} = 0.2~\rm{ns}$ and an energy
of $250.0~\rm{GeV}$, this corresponds to a mean decay length of
$10.07~\rm{cm}$. A second signal sample is generated with
$\tau_{\tilde{\chi^0_1}} = 2.0~\rm{ns}$.

At the ILC $500~\rm{fb}^{-1}$ integrated luminosity at $\sqrt{\rm{s}}
= 500~\rm{GeV}$ with \mbox{$+ 80~\%~\rm{e}^-$} and \mbox{$-
  60~\%~\rm{e}^+$} polarisation, $217\cdot 10^3$ signal events,
corresponding to a cross section of $\sigma = 433.5 \pm 0.6~\rm{fb}$
are expected. The topology, two high energy photons and missing
energy, might be mimicked by at least $5.3 \cdot 10^6$ SM back\-ground
events including photons (and neutrinos). This is consistent with a
signal to back\-ground ratio of $\rm{S} : \rm{B} \approx 1 : 24.3 $.
It can be enhanced to $\rm{S} : \rm{B} \approx 0.9 : 1$ for the $\tau
= 0.2~\rm{ns}$, and $\rm{S} : \rm{B} \approx 1.0 : 1$ for the $\tau =
0.2~\rm{ns}$ sample, respectively, with a cut based selection
explained in~\cite{analysis-note}.

The neutra\-lino mass can be determined from the photon energy
distribution: $\rm{m}_{\tilde{\chi^0_1}} = \frac{1}{2} \sqrt{\rm{s}
  \mp (4 \cdot \rm{E}^{\gamma}_{\rm{min,max}} - \sqrt{\rm{s}})^2} $.
The reconstructed mass is $\rm{m}_{\rm{reco}} = 146.0 \pm
2.2~\rm{GeV}$, while one obtains $\rm{m}_{\rm{MC}} = 154.2 \pm
1.5~\rm{GeV}$, using MonteCarlo information.

The neutra\-lino flight distance can be calculated according to $
\lambda = |\vec{\rm{cog}}| \cdot
\frac{\sin{\phi}}{\cos{\psi}}$~\cite{GMSBatILC-2}. Here $\psi$ is the
angle between the shower centre of gravity $\vec{\rm{cog}}$ and the
principal axis of inertia. The decay angle $\phi$ between neutralino
and photon is reconstructed from the measured photon energy
$\rm{E}_{\gamma}$: $ \cos{\phi} =
\frac{\rm{E}_{\tilde{\chi}^0_1}}{\rm{p}_0} -
\frac{\rm{m}^2_{\tilde{\chi^0_1}}}{2 \cdot \rm{p}_{\tilde{\chi}^0_1}
  \rm{E}_{\gamma}} $, where $\rm{p}_{\tilde{\chi}^0_1}$ corresponds to
the neutra\-lino momentum. The lifetime obtained by this
reconstruction method, as plotted in Figure~\ref{fig:gmsb_results} is
$\tau_{\rm{reco}} = 2.02 \pm 0.02~\rm{ns}$ and $\tau_{\rm{MC}} = 1.9
\pm 0.02~\rm{ns}$ for the $\tau_{\rm{true}} = 0.2~\rm{ns}$ sample, and
$\tau_{\rm{reco}} = 0.333 \pm 0.003~\rm{ns}$ and $\tau_{\rm{MC}} =
0.48 \pm 0.009~\rm{ns}$ for the $\tau_{\rm{true}} = 0.2~\rm{ns}$
sample.

Within this analysis 100 cm decay length can be well measured, while
10 cm decay could not be reconstructed with the ECAL only.

%%\begin{figure}[ht] 
%%  \centering     
 %%   \includegraphics[width=7.5cm]{gmsb_02ns.pdf}
  %%  \includegraphics[width=7.5cm]{gmsb_2ns.pdf}
   %%\caption{Neutralino lifetime
   %% determination for neutra\-linos with (a) 0.2 ns and (b) 2.0 ns
   %% input life\-time.
  %%\label{fig:gmsb_results}}
%%\end{figure}



==> performance/physics_higgs_mass_mat.tex <==
The precise determination of the properties of the Higgs boson is one of the main
goals of the ILC. Of particular importance are the Higgs boson mass, $\mH$, and its branching 
ratio. Fits to current Electroweak data\cite{bib:lepewwg} and direct limits from searches
at LEP and at the Tevatron favour a relatively low value for $\mH$. Studies of the 
measurments of $\mH$ and the Higgs branching ratios are presented below. In both cases,
a data sample of 250\,fb$^{-1}$ at $\roots=250$\,GeV is assumed and the Higgs mass is
taken to be 120\,GeV. For this case the dominant Higgs production process is
that of Higgsstrahlung, $e^{+}e^{-} \rightarrow HZ$. All results are based in
the full simulation of the ILD detector and full reconstruction of the generated
events.

At the ILC the the best measurement of the Higgs boson mass is obtained from
$\Zzero\Higgs\rightarrow\epem X $ and
$\Zzero\Higgs\rightarrow\mpmm X $ where $X$ represents the Higgs decay products.
For these channels the Higgs mass is most precisely determined from the mass distribution
of the system recoiling against the $\Zzero$. This is one of motivations for the 
momentum resolution requirements for an ILC detector. The $\mmX$-channel yields the
most precise measurement as the $\eeX$-channel suffers from larger experimental uncertainties 
due to Bremsstrahlung from the electrons and the larger background from Bhabha scattering events.
The study is performed for two electron/positron beam polarisations:  $e^-=+80\%$, $e^+=-30\%$ and 
$e^-=+80\%$, $e^+=-30\%$. In the simulation, the energy spread for both incoming beams 
is 0.3\%. 

The first stage in the event selection is the identification of leptonically decaying $\Zzero$ bosons.
Candidate lepton tracks are required to be well-measured tracks with transverse momentum 
$p_T>{\rm15\,GeV}$. Lepton identification is performed using the associated calorimetric 
information resulting in a identification efficiency of 95.4\,\% for muons and 98.8\,\% for electrons.
Candidate $\Zzero$ decays are identified from opposite charged pairs of identified leptons
within a mass window around $\mZ$. Background from $\Zzero\rightarrow\lplm$ is rejected
using cuts on transverse momentum of the di-lepton system, $p_T>20$\,GeV and the 
acoplanarity of the two lepton tracks, $0.2<\theta_{acop}<3.0$. Additional 
cuts reject $\Zzero\rightarrow\lplm$ events with initial and final state radiation.
The background from $e^{+}e^{-} \rightarrow \Zzero\Zzero$, $e^{+}e^{-} \rightarrow \WpWm$ 
is reduced by a multi-variate likelihood analysis based on the acoplanarity, the polar angle, 
the transverse momentum and the invariant mass of the di-lepton system.

\begin{figure}[!h]
\centering
\includegraphics[width=7.5cm]{fit_mu_mi_lr_gpet.pdf}
\includegraphics[width=7.5cm]{fit_el_mi_lr_gpet.pdf}
\caption{Results of the model independent analysis of the Higgs-strahlungs Process 
$\epem \rightarrow \Higgs\Zzero$ in which a) $\Zzero\rightarrow\mpmm$ and b) $\Zzero\rightarrow\epem$. 
The results are shown the $e^+=+80\,\%$, $e^-=-30\,\%$ beam polarisation. 
\label{fig:fit_ppme_gpet}}
\end{figure}
The reconstructed recoil mass distributions, calculated assuming the $\Zzero\Higgs$ is produced with
four-momentum $(\roots,\bf{0})$, are shown in Figure~\ref{fig:fit_ppme_gpet}.
The combination of signal and background is fitted using a function which assumes a 
Gaussian-like signal and that the background can be approximated by a polynomial function. 
The results of the fit for the $\mH$ and the $\sigma(\epem\rightarrow\Zzero\Higgs$ 
are listed in Table~\ref{tab:mirst}. Also shown are the results obtained when assuming the 
Standard Model decay modes and branching fractions. In this case, labelled ``Standard Model'
the background can be further reduced by requiring charged tracks in addition to those generated by 
the $Z$-Boson decay products. 

\begin{table}[!h]
\centering 
\begin{footnotesize}
\begin{tabular}{|l|l|l|r|rr|}
\hline
Analysis &Polarisation ($e^-,e^+$) & Channel & $\sigma_{\mH}$ & \multicolumn{2}{c|}{Cross section}\\\hline
\multirow{4}{*}{Model Independent}
&\multirow{2}{*}{$(+80\,\%,\, -30\,\%)$} & $\mmX$ &   90\,MeV &  $\pm0.50$\,fb & (7.0\,\%)   \\\cline{3-6}
&                       & $\eeX$ &  182\,MeV &  $\pm0.87$\,fb &(12.2\,\%)   \\ \cline{2-6} 
&\multirow{2}{*}{$(-80\,\%,\, +30\,\%)$} & $\mmX$ &   85\,MeV &  $\pm0.70$\,fb & (6.6\,\%)   \\\cline{3-6}
&                       & $\eeX$ &  128\,MeV &  $\pm0.90$\,fb & (8.3\,\%)   \\ \hline
\multirow{4}{*}{Standard Model} 
&\multirow{2}{*}{$(+80\,\%,\, -30\,\%)$} & $\mmX$ &   84\,MeV &  $\pm0.45$\,fb & (6.4\,\%)   \\ \cline{3-6}
&                       & $\eeX$ &  204\,MeV &  $\pm0.74$\,fb &(10.3\,\%)   \\ \cline{2-6} 
&\multirow{2}{*}{$(-80\,\%,\, +30\,\%)$} & $\mmX$ &   77\,MeV &  $\pm0.55$\,fb & (5.4\,\%)   \\ \cline{3-6}
&                       & $\eeX$ &  135\,MeV &  $\pm0.85$\,fb & (8.0\,\%)   \\ \hline
\end{tabular}
\end{footnotesize}
\caption{Expected statistical uncertainties on $\mH$ from the recoil mass distribution in the
           in Higgs-strahlung events where the $Z$ decays into either $\epem$ or $\mpmm$.
           Results are listed for both the model independent and Standard Model analyses.
           Also listed are the experimental uncertainties on the Higgs-strahlung 
           cross section,
           $e^{+}e^{-}\rightarrow \Higgs\Zzero \rightarrow \mmX$ and 
           $e^{+}e^{-}\rightarrow \Higgs\Zzero \rightarrow \eeX$.
           The results are shown for two different beam polarisations. 
\label{tab:mirst}}
\end{table}

From Figure~\ref{fig:fit_ppme_gpet} and Table~\ref{tab:mirst} the following 
conclusions can be drawn: i) using the recoil mass distributions in the $\mmX$ and $\eeX$ final
states, the $\mH$ can be determined with a statistical uncertainty of about 70\,MeV 
and the Higgs-strahlung cross section to a precision of about 5\%; ii) the precision 
obtained in the $\eeX$ channel is approximately a factor two worse than that obtained from
the $\mmX$ channel. This is due to bremsstrahlung from the final states electrons in the 
detector material and the large potential background from Bhabha scattering; 
iii) in the $\eeX$ channel the $\mH$ uncertainty depends strongly on the 
beam polarisation, this is due to the reduction in the large Bhabha scattering
background, e.g. the signal to background ratio in the recoil mass window
$110-150$\,GeV is $\sim$0.4 for the $(e^-=+80\,\%,\, e^+ =-30\,\%)$ polarisation and
$\sim$0.2 for the $(e^-=-80\,\%,\, e^+ =+30\,\%)$ polarisation; and 
iv) for the current analysis, the reduction in background in the Standard Model analysis 
compared to the Model Independent analysis reduces the error on $\mH$ by $\sim10\,\%$.  
 

%%The remaining signal over background ratio $S/B$ is around 0.5 for the $e^-_{R}=+80\%$ $e^+_{L}=-80\%$ 
%%polarisation mode and around 0.3 for the $e^-_{L}=+80\%$ $e^+_{R}=-80\%$ polarisation mode. 
%%Apart from 'usual' kinematic and acceptance cuts the background can be successfully suppressed by 
%%making use of the excellent particle separation capabilities of the ILD detector when for instance 
%%reconstructing electrons from converted radiative photons which have been misidentified and muons.
%% The remaining background is dominantly given by the concurring processes
%% The applied procedures for signal selection and background suppression leads to a reduction 
%%of the signal sample between 40\% and 60\% while the 
%%item $eeX$: The situation is less distinct for this decay channel of the $Z$-Boson. Although also in this mode the signal from the Higgs Boson is clearly visible the precision of the
%% result is reduced by a factor two. This caused by bremsstrahlung when the final states electrons interact with the detector material and by remaining non-reducible background given by Bhabha scattering. Note, however that the cross section of Bhabha scattering is six order of magnitudes larger than that of the Higgs Strahlungs Process. This is reduced such that the remaining signal over background ration is around 0.4 for the $e^-_{R}=+80\%$ $e^+_{L}=-80\%$ and around 0.2 for the  $e^-_{L}=+80\%$ $e^+_{R}=-80\%$ polarisation mode.
%%\end{itemize}
%\subsection{Higgs Decays into Standard Model Particles}
%%If the study is performed assuming that the Higgs Boson can solely decay into final states favoured by the Standard Model, hence introducing a
%%{\it Model Dependency} the background can be further reduced by requiring charged tracks in addition 
%%to those generated by the $Z$-Boson decay products. 
%%\begin{figure}[!h]
%%\centering
%%\includegraphics[width=7.5cm]{fit_mu_sm_lr_gpet.pdf}
%%\includegraphics[width=7.5cm]{fit_el_sm_lr_gpet.pdf}
%%\caption{Results of the Higgs Strahlungs Process $e^{+}e^{-} \rightarrow HZ $ in which the Z decays into a muon pair   ($\mu\mu X$, left) and into an electron-positron pair ($eeX$, right) after introducing a {\it Model Dependency} as suggested by the Standard Model. The results are displayed for the polarisation mode $\rm{e^+_Re^-_L}$ of the incoming beams.
%%\label{fig:fit_sm_ppme_gpet}}
%%\end{figure}
%%From Figure~\ref{fig:fit_sm_ppme_gpet} and Table~\ref{tab:smrst} it can be deferred that in particular the precision of the mode in which the $Z$-Boson decays
%%into electron-positron pairs benefit considerably from this further assumption as it allows for the full suppression of the
%%Bhabha background. The precision is increased by 25\% which is true for both, the Higgs Mass determination and the cross section measurement. 
%%\begin{table}[!h]
%%\centering 
%%\begin{footnotesize}
%%\begin{tabular}{|l|l|l|l|l|}
%%\hline
%%Polarisation ($e^-,e^+$) & Channel & $\mH$ /GeV & Cross section /fb \\%%
%%
%%\hline
%%$(+80\,\%,\, -30\,\%)$ & $\mmX$ & $119.951 \pm 0.084$ & $6.98 \pm 0.45$ (6.4\,\%)\\
%%                       & $\eeX$ & $119.713 \pm 0.204$ & $7.18 \pm 0.74$ (10.3\,\%)\\
%%\hline
%%$(+80\,\%,\, -30\,\%)$ & $\mmX$ & $119.905 \pm 0.077$ & $10.26 \pm 0.55$ (5.4\,\%)\\
%%                      & $\eeX$ & $119.871 \pm 0.135$& $10.67 \pm 0.85$ (8.0\,\%)\\
%%\hline
%%\end{tabular}
%%\end{footnotesize}
%%\caption{Results of the analysis of the Higgsstrahlungs process, assuming the
%%         Standard Model branching ratios of the Higgs boson, where the  
%%          $Z$ decays 
%%          into either $\epem$ or $\mpmm$. The results are shown for
%%          two different beam polarisations.
%%          \label{tab:smrst}}
%%\end{table}
 
\subsection{Influence of Beam Energy Spread} 

The width of the peak of the recoil mass distribution is predominantly a convolution 
of detector response and spread of the energies 
of the incoming electron and positron beams. For the $\mmX$ channel the contribution
from the detector response is primarily due to the momentum resolution, whereas for
the $\eeX$ channel bremsstrahlung from to the interaction of the final electrons with the 
detector material dominates. 
The beam energy spread depends on the accelerator design. In the simulation, the rms beam energy 
spread is taken to be $0.3\,\%$ for both the electron and positron beams.
%It is natural to ask whether it is the detector response or the beam energy spread
%that dominates the width of the recoil mass peak. 
Figure~\ref{fig:mh_gen_sim} 
shows the recoil mass spectrum for the $\mmX$ channel obtained from the generated 
four momenta of muon pair compared to that obtained from the reconstructed momenta.
The detector response leads only to a relatively small additional broadening of 
the recoil mass peak; the width of the peak  {\bf HOW IS THIS DEFINED} increases from 
730\,MeV to 870\,MeV. Hence it is concluded that the dominant contribution to the 
observed width of the $\mmX$ recoil mass distribution arises from the 
incoming beams rather than the response of the ILD detector.. 
 

\begin{figure}[h]
\centerline{\includegraphics[width=10cm]{mh_mu_gen_sim}}
\caption{The Higgs recoil mass distribution in the $\mmX$ channel obtained from the generator level and
          reconstructed muon pair momenta. \label{fig:mh_gen_sim}}
\end{figure}



==> performance/physics_smuons.tex <==
SUSY may provide a rich 
spectrum of kinematically 
accessible 
particles at the ILC operating at $\roots=500$\,GeV, 
for example the production of gauginos and sleptons with masses below 
$250\,\mathrm{GeV}$. The signals for new physics may consist
of a complex mixture of dominant and sub-dominant processes, often with 
the identical visible final states. In this case it may be
necessary to measure the properties of the new particles
simultaneously~\cite{smuon_ref1}. 

Here we consider the final
state consisting of two muons and missing energy in
mSUGRA SUSY with the $SPS1a^{'}$ parameters:
$M_{0}=70\,\rm{GeV}$, $M_{1/2}=250\,\rm{GeV}$, $A_{0}=-300\,\rm{GeV}$,
sign$(\mu)=+1$, and $\tan\beta=10$.
The $\chi_{1}^{0}$, $\chi_{2}^{0}$, and $\tilde{\mu}_{L}$ masses can be 
measured from
$\chi_{2}\chi_{1}\rightarrow \mu\mu\chi_{1}^{0}\chi_{1}^{0}$ ($\sigma = 4.1$\,fb) and
$\tilde{\mu}_{L}\tilde{\mu}_{L}\rightarrow \mu\mu\chi_{1}^{0}\chi_{1}^{0}$
($\sigma = 54$\,fb).
The potential precision for these measurements at the
ILC operating at $\sqrt{s}=500\,\mathrm{GeV}$ is studied
using the full ILD detector simulation and reconstruction chain. 
For the main result a beam polarisation of $P(e^+,e^-) = (+30\,\%,-80\,\%)$ 
is assumed.


The SUSY signal considered here is characterised by two hard muons
($E_{\mu}>40$\,GeV) and missing energy. Energetic muons are identified with $95\,\%$ efficiency using 
track, HCAL and muon chamber information. The momentum 
resolution of the selected muons is $\sigma_{p_{T}}/p \sim 3 \times 10^{-5}$.
The signal events are selected using the following variables: the missing energy,
$E_{miss}$; the invariant mass of the di-muon system, $m_{\mu\mu}$;
the invariant mass of the invisible system,
$m_{\mu\mu}^{miss}$; the transverse momentum, $p_{T}$;
and the direction, $\theta_\beta$, and speed, $\beta$, of the
Lorentz transformation from the laboratory frame to the centre of mass
frame of the di-muon system. Cuts on these variable are used to define
$\tilde{\mu}_{L}\tilde{\mu}_{L}\rightarrow\mu\mu\chi_{1}^{0}\chi_{1}^{0}$ and
$\chi_{2}\chi_{1}\rightarrow \mu\mu\chi_{1}^{0}\chi_{1}^{0}$ event samples. 


The masses of the $\chi_{1}^{0}$ and of the $\tilde{\mu}_{L}$ are
measured from the kinematic edge of the momentum distribution of the
muons in the decay chain $\tilde{\mu}_{L}\tilde{\mu}_{L}\rightarrow
\mu\mu\chi_{1}^{0}\chi_{1}^{0}$~\cite{smuon_ref2}. 
%%The signal is selected with the
%%following cuts: 
%%$200\,\rm{GeV}<E_{miss}<430\,\rm{GeV}$,
%%$m_{\mu\mu}>40\,\rm{GeV}$, 
%%reject events with $0.1\,\pi<\theta_{\beta}<0.9\,\pi$ or
%%$80\,\rm{GeV}<m_{\mu\mu}<120\,\rm{GeV}$.
%%Two beam polarisations are considered,
%%$P(e^+,e^-) = (+30\,\%,-80\,\%)$ and 
%%$(+60\,\%,-80\,\%)$.
%% The cuts select 
%% $n_{s}=15100$ signal and $n_{b}=15700$ background 
%%events, where the numbers in brackets refer to the
%%$(+30\,\%,-80\,\%)$ polarisation. 
%%{\bf COULD WE QUOTE WHAT INTEGRATED LUMINOSITY IS REQUIRED TO GET A 
%%     5 SIGMA SIGNAL ? }
%%In both cases  significance largely above
%%$5\sigma$ is reached. 
The muon momentum distribution for the selected events are
shown in Figure~\ref{fig:smu}a. The kinematic edges of the signal, 
at 32\,GeV and 151\,GeV are fitted with a step function yielding
measurements of the masses of the $\chi_{1}^{0}$ (97.71\,GeV) 
and the $\tilde{\mu}_{L}$ (189.87\,GeV)
with statistical uncertainties of $1.40\,\%$ 
and 0.27\,\% repectively. 
The signal cross section is determined,
from the number of selected events
accounting for the background contribution,
with a relative statistical 
uncertainty of $2.53\,\%$. 
The sharpness of the kinematic edges, and consequently the 
mass measurements, are limited by
beamstrahlung rather than the track momentum resolution; it
is estimated that for the lowP option, the uncertainty in the $\chi_{1}^{0}$
mass would be a factor 2 worse.

\begin{figure}[t]
\centering
\includegraphics[width=7.5cm]{LOI_smu.pdf}
\includegraphics[width=7.5cm]{LOI_chi.pdf}
\caption{\label{fig:smu} (a) Distribution of the momentum of the $\mu^{+}$ in 
the laboratory frame after the selection of the $\tilde{\mu}_{L}\tilde{\mu}_{L}$ 
pair candidates. The total observed signal and the backgrounds (SUSY and SM) 
are reported. The mass of the $\chi_{1}^{0}$ is measured from the 
kinematic edges of the distribution of the momentum of the di-muons.
There are two entries for each event. 
(b) Fitted $m_{\mu\mu}$ spectrum. The kinematic edge corresponding to 
the $\chi_{2}^{0}\rightarrow \tilde{\mu}_{R}\mu$ can be extracted from the 
fit on top of the left tail of the $Z$ peak. Both plots are shown for
a beam polarisation of -80\,\%, 60\,\% and correspond to an integrated luminosity
of 500\,fb$^{-1}$.}
\end{figure}

The $\chi_{2}^{0}$ mass is determined from the kinematic edge of
the di-muon mass distribution in the decay chain
$\chi_{2}\chi_{1}\rightarrow \mu\mu\chi_{1}^{0}\chi_{1}^{0}$~\cite{smuon_ref2}. 
%%The cuts used are:
%%$355\,\rm{GeV}<E_{miss}<395$\,GeV,
%%$p_{t}>40\,\rm{GeV}$, $m_{\mu\mu}>40$\,GeV 
%%$m_{\mu\mu}^{miss} < 80$\,GeV or  
%%$m_{\mu\mu}^{miss} > 100$\,GeV,
%%$0.1\,\pi<\theta_{\beta}<0.9\,\pi$.  
The
resulting distribution of $m_{\mu\mu}$ after the selection 
is shown in Figure~\ref{fig:smu}b.  
The kinematic edge of the signal is visible below the $Z$ peak.
A fit to the region $40\,\rm{GeV}<m_{\mu\mu}<85\,\rm{GeV}$ is used
to determine the mass of the
$\chi_{2}^{0}$ (183.89~GeV). In this region 
there are 490 signal events and 2500 background events; the 
statistical significance of the excess corresponds 9 standard deviations
and the $\chi_2^0$ mass resolution obtained is $1.41\,\%$. 
%%For $60\%$ polarizationt he cross section of the
%%process can be measured within the $95\,\%$ C.L. band
%%$(3.75,5.57)$\,fb. 

The above study demonstrates that dominant and sub-dominant SUSY 
processes with identical final states can be disentangled successfully 
in the $SPS1a^{'}$ scenario with the ILD detector concept
and that the masses of SUSY particles can be measured to ${\cal O}(1\,\%)$.
A higher positron polarization yields significantly 
improved precision, particularly for $\chi_2\chi_1$ production where a
positron polarisation of $60\,\%$ rather than $30\,\%$  results in
50\,\%  more signal events for a relatively small increase in
background. 



==> performance/physics_stau_mass.tex <==


\subsection{Stau Mass}

% As mentioned in the introduction,
% SUSY itself poses a background problem in the $\tau$ analysis,
% and it is therefore needed to run the ILC at the
% polarisation that minimises the background.
% For
% 100 \% left  e$^-$ polarisation and 100 \% right e$^+$ polarisation,
% the cross-sections for $\XN{2} \XN{2}$ and $\XP{1} \XM{1}$ are
% several hundred fb, and the branching ratios to $\stau$ is above
% 50 \%. With the opposite polarisation, however, these cross-sections
% will almost vanish.
% Hence, these channels were studied assuming
% 80 \% right  e$^-$ polarisation and 60 \% left e$^+$ polarisation.

% As the $\gamma \gamma$ background poses another challenge
% for the $\tau$ channels, quite strong criteria must be applied:
% A correlated cut in $\rho$ (the transverse momentum of the jets
% wrt. the thrust axis, in the projection perpendicular to the beam)
% was also done: $\rho > 3\sin{\theta_{acop}}+1.7$.
% To further reduce the $\gamma\gamma$ background to
% acceptable levels, it was demanded that there be no significant
% activity in the BeamCal, and that the $\phi$ angle of the
% missing momentum was not in the direction of the
% incoming beam-pipe.

The $\stau$ mass can be extracted from the end-point of the 
spectrum of E$_{jet}$, which is equal to  $E_{\tau,max}$, 
and the $\XN{1}$ mass, known eg. from the
$\smul$ analysis above. In principle, the maximum of
the spectrum is at $P_{\tau,min}$, so that the $\stau$ can
be used to find $\MXN{1}$ as well, but due to the large
$\gamma \gamma$ background, the maximum is quite hard
to observe. 

\begin{figure}
\centering
\includegraphics[width=6cm]{mass-fit-stau-sps1a.pdf}
\caption{Jet Energy spectrum. Black: total spectrum; Red: total background;
Green: SUSY background. Blue line: fit to background (the solid
part is the fitted function, the dashed is it's extrapolation into
the signal region); Read line: fit to total spectrum minus
fitted background.\label{tab:staumass_jetspect}}
\end{figure}

To extract the signal in order to determine the end-point, 
the same cuts were used as for the $\tau$-polarisation
analysis, except that no selection of specific
decay-modes was performed. Two additional cuts replaced
the decay-mode specific cuts: The mass of both jets
was required to be less than 2\,GeV, and 
$|\cos{\theta_{missing p}}|$ was required to be less
than 0.75.
% the
% following cuts were applied:
% $E_{miss} \in [430,490] ~\GeV$, 
% $M_{jet} < 2 ~\GeVcc$,
% $\theta_{jet}$ above 20 degrees,
% $\theta_{acop} < 160$ degrees,
% $\theta_{acol} \in [80,170]$ degrees,
% $|\cos{\theta_{missing p}}| < 0.9$, and
% charge of each jet = $\pm 1$.
% In addition, the anti-$\gamma\gamma$ cut described above was applied.
After these cuts, the SM background was 1143 jets, the SUSY
background was 3172, while 16811 signal jets remained (12.0 \%
efficiency). Fig.~\ref{staumass:jetspect} shows that background
around the end-point is
quite small, and also that the turn-over point
(expected to be at $P_{\tau,min} = 2.2$\,GeV)
is too distorted by the cuts to be useful.
The remaining background close to the end-point - in the range 
$30 - 70$\,GeV - was found to be
well described by an exponential, and it was fitted in the
signal-free region above 46\,GeV. The background-fit was
subtracted from the observed spectrum, and a straight line
fit was done in the range $30 - 41.5$\,GeV. 
The result of the simulaneous fit of background and signal 
is $\mstone = 108.08 \pm 0.10$\,GeV.
% where the uncertainty of the background has been added in quadrature.
(The true value in SPS1a' is $\mstone = 107.86$\,GeV.)
However, this result assumes that $\MXN{1}$ is known. At this
model-point, the derivative of $\mstone$ wrt. $\MXN{1}$ is 1.3,
so the actual error on $\mstone$ is 100\,MeV $\oplus$ 
1.3$\sigma_{\MXN{1}}$. Assuming that all smuons and selectrons
will yield a similar result on $\sigma_{\MXN{1}}$ as
the result quoted above for the $\smul$, one could expect
that $\sigma_{\MXN{1}} \approx 250$\,MeV, and consequently that
$\mstone = 108.08 \pm 0.33\,$GeV.
 


==> performance/physics_staus.tex <==

\begin{figure}
\includegraphics[height=5cm]{Initial_Stau_Spectrum.eps}
\includegraphics[height=5cm]{Stau_Spectrum.eps}
\caption{ \label{tab:}}
\end{figure}

% The measurement of the degree of tau polarisation $P_\tau$ in $\tilde{\tau}_1$ decays can give a insight to various aspects of 
% the supersymmetric theory. Depending on the SUSY point $P_\tau$ is sensitive to the ratio of the Higgs vacuum expectation values 
% $\tan \beta$ and via that to the trilinear couplings $A_\tau$ \cite{}, the mixing parameters in the $\tilde{\tau}$ sector \cite{} 
% and the neutralino mixing.
%In this mSUGRA SUSY scenario the $\tilde{\tau}$ is the NLSP with $\unit[m_{\tilde{\tau}}=107]{GeV}$, the neutralino $\chi_1$ is the LSP with a mass of $\unit[97]{GeV}$ and $\tan \beta = 10$ which results in an expected degree of polarisation is $P_\tau = \unit[97]{\%}$.

The SUSY process of stau pair production provides a number of challenges:
it requires precision tracking of relatively low momentum particles, 
good particle indentification, high hermeticity of the detector, 
and low machine background.
Of particular importances is the measurement of tau polarisation, $P_\tau$, 
in $\tilde{\tau}_1$ decays. This gives which direct access to the mixing of mass in interaction
eigenstates in the stau sector, and thus provides sensitivity to a number of SUSY parameters.
This study probes the possibility of measuring, $P_\tau$, 
for SUSY parameter point SPS1a' with $L=500\,{fb^{-1}}$. In this scenario $P_\tau = 97\,\%$
and is best determined in the process 
$e^+e^- \rightarrow \tilde{\tau}\tilde{\tau} \rightarrow \chi_1 \tau \chi_1 \tau$. The 
cross section is maximum for a beam polarisation with left handed positrons and right handed 
For this polarisation, $\tilde{\tau}_1$ pair production has the highest cross-section in 
the SUSY sector and the background from other
SUSY and SM background processes is minimised.
{\bf WHAT POLARIZATION WAS USED FOR THIS STUDY +80, -30 ? }


The decay mode $\tau \rightarrow \pi \nu_\tau$ has an expected yield of $\sim$17500 charged pions and % in $L = 500\,{fb^{-1}}$ and
allows determination $P_\tau$ via a measurement of the pion energy spectrum. 
For positive $P_\tau$ the spectrum has a characteristic triangular shape which is sensitive to $P_\tau$ and
theoretically described. 

In the final state, the signal pion appears isolated with a second tau jet of five charged tracks at most. 
Kinematic constrains limit the energy of both to $< 43\,$GeV. 
%the taus %is determined by the $\chi_1$ to $\tilde{\tau}$ mass difference and %limited to $\unit[\sim 43]{GeV}$.
Signal pion candidates are searched in events which feature $400\,$GeV of missing energy and vanishing total charge.
This extraction yields 12600 signal pions which have been identified as pions by exploiting calorimeter and 
d$E$/d$x$ information. 

Curial backgrounds are two photon processes, especially when a tau pair is present in the final state 
(Figure \ref{Initial_Pion_Spectrum}). These backgrounds are 
reduced by the veto of the beam calorimeter and a cut on the transverse momentum to a thrust axis in the transversal plane. 
In the further selection, the invariant mass of everything in the event except ths signal pion candidate is 
constraint to $\le2.5\,$GeV, signal candidates found the forward region excluded $|\cos \Theta| > 0.9$ 
and a acoplanarity angle $\Phi_\text{acoplan} \ge 85^\circ$ requested. 
Due to the hole in the beam cal around the incoming beam pipe, a certain region in $\Phi$ must be rejected: 
$\Phi \le 110^\circ$ or $\Phi \ge 250^\circ$ (for details see \cite{ref:Schade}.
 
The selection identifies 2350 signal pions with a background of 500. 
The initial pion spectrum is reconstructed by subtracting the remaining background in a parametrised 
form and application of an energy dependent efficiency correction. 
Besides $P_\tau$ the shape of the spectrum is also influenced by the luminosity spectrum of the machine. 
This effect is folded into the fit function.
Figure \ref{Final_Pion_Spectrum} shows the reconstructed data points together with the fit.

The study of the robustness of the method and detector parameters shows, that an accuracy of in the range  
$\Delta P_\tau = 15\,\%$ seem realistic.




==> performance/physics_wimp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Model-independent WIMP search: $e^+e^- \rightarrow \chi\chi\gamma$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A possible candidate for Dark Matter constituents are Weakly Interacting Massive Particles (WIMPs).
If they can pair annihilate at least to a fraction into $e^+e^-$ pairs, the reversed process can be detected at the ILC when the two WIMPs are accompanied by photon radiation from the incoming particles. In these events, the photon recoil mass has a characteristic onset, depending in location and shape on the mass and spin of the WIMP candidate.

However, there is a large irreducible background from neutrino pair production accompanied by ISR.
Within the Standard Model Monte-Carlo sample processed for all LoI studies, matrix elements with up to three photons in the final state have been taken account, plus one additional (soft) ISR photon from each beam. Therefore excellent photon energy and angle resolution are required in order detect a clear edge from the signal in the photon energy spectrum above a huge background. 

Assuming that the total cross-section for WIMP pair annihilation into Standard Model fermion pairs, $\chi\chi \rightarrow f\bar{f} $, is known from cosmological observations, the ILC sensitivy can be expressed in terms of the WIMP pair branching fraction into $e^+e^-$, $\kappa_e$. Besides their mass and $\kappa_e$ values, the WIMPs may have different spins and helicity structure as well as different dominant partial waves in the annihilation process. The analysis has been performed for an integrated luminosity of 500~fb$^{-1}$ at a  center-of-mass energy of $E_\mathrm{CM} = 500$~GeV, which beam polarisations of $P(e^+,e^-) = (-30\%,+80\%), (-60\%,80\%)$ as well as without positron polarisation.

The left panel in figure~\ref{fig:sensitivity} shows the 95\% CL sensitivity on $\kappa_e$ as a function of the WIMP mass for three different types of WIMPs: xxx, yyy, zzz, meaning that $\kappa_e$ values above the curves could be excluded at 95\% CL. In the right panel, the impact of different beam polarisations is shown for a WIMP with  helicity and parity conserving couplings. 
Only WIMP masses above 100~GeV are considered here, since lower mass WIMPs would be produced with relativistic velocities at $E_\mathrm{CM} = 500$~GeV, so that the normalisation to the non-relatovistic cosmological annihilation cross-section would not hold anymore. In general, $\kappa_e$ values of 0.1 are accessible for WIMP masses of up to about 200~GeV.

\begin{figure}
\begin{center}
%\epsfig{figure=kappa_severalWIMPS_pol3080.eps,width=6cm}
%\epsfig{figure=kappa_oneWIMPS_severalpols.eps,width=6cm}
\end{center}
\label{fig:sensitivity}
\caption{Left: 95\% CL sensitivities in terms of the WIMP pair branching fraction into $e^+e^-$, $\kappa_e$ for three different WIMP types as a function of the WIMP mass, assuming a beam polarisation of $P(e^+,e^-) = (-30\%,+80\%)$. Right: 95\% CL sensitivity on $\kappa_e$ for three different beam polarisations.}
\end{figure}



==> performance/tracking.tex <==
%%28/03/2009 M.Thomson
The tracking system of the ILD detector concept consists
of a vertex detector (VTX) and a large volume TPC, complemented
by additional Silicon tracking layers (FTD/SIT). 
In addition, in the LDC-based models,
silicon tracking layers immediately outside the TPC are considered 
(ETD and SET). The dependence of the performance of the 
tracking system on the magnetic field and detector
size was an important consideration in optimising the 
ILD. Considerations of momentum
resolution favour a larger detector and higher 
magnetic field. As discussed above, a higher magnetic field also
allows the first layer of the vertex detector to be
closer to the interaction point (IP).
The optimisation of the tracking system is, again, a 
balance between the magnetic field and detector radius.
The parameter space spanning the LDC (smaller $R$, higher $B$-field)
and GLD (larger $R$, lower $B$) concepts is investigated
using the six detector models summarised in Table~\ref{tab:optdetparameter}.

\subsection{Momentum resolution}

Figure \ref{fig:mreso_jupiter}(a) shows the $1/p_\mathrm{T}$ resolution, 
as a function of $p_{\mathrm{T}}$, for single muons in 
the GLD, GLDPrime and GLD4LDC models. The results were 
obtained using the Satellites Kalman Filter 
(Section~\ref{sec:optimisation-simulation-jsf}). 
Figure \ref{fig:mreso_jupiter}(b) shows the relative $1/p_\mathrm{T}$ resolution compared
to the average of three detector models at a particular value of
$p_\mathrm{T}$, plotted as a function of $p_{\mathrm{T}}$.
Above approximately 50 GeV, the resolution obtained with the GLD4LDC model 
is $\sim$5\,\% worse than the larger detector models due to the
shorter lever arm 
of the TPC. For lower energy tracks the situation is reversed with the
higher magnetic field resulting in the resolution for 4\,T being $\sim$10\,\% 
better than for 3\,T. Similar results were obtained with the LDC-based
models using Mokka and MarlinReco (Section~\ref{sec:optimisation-simulation-mokkamarlin}).
The relative performance does not depend strongly on angle.
The differences in resolution for the
range of $B$ and $R$ considered are small ($\lesssim10$\,\%) 
compared to those arising from different
layouts for the tracking system and the point resolutions of the components. 
For example, the use of hits in the silicon external tracker (SET) 
outside the TPC in the LDCPrime model improves the momentum resolution by 
15\,\% assuming an SET  $r\phi$ hit resolution of 4\,$\mu$m.


\begin{figure} 
\begin{center}
\includegraphics[width=7.0cm]{mgld.pdf}
\includegraphics[width=7.0cm]{mgldratio.pdf}
\caption[Transverse momentum resolution versus momentum.]{(a) $\sigma_{1/p_\mathrm{T}}$ for single muon tracks at 
   $90^\circ$ to the beam axis, as a function of transverse momentum, for the
   GLD, GLDPrime, and GLD4LDC models; and (b) the ratio of $\sigma_{1/p_\mathrm{T}}$ to the 
   average of the 
   three detector models as a function of transverse momentum. To avoid the TPC central
   membrane the generated muons were displaced from the IP by a few centimetres.}
\label{fig:mreso_jupiter}
\end{center}
\end{figure}

%%\begin{figure}
%%\centering
%%\includegraphics[width=5cm]{Kappa1GeV.pdf}
%%\includegraphics[width=5cm]{Kappa10GeV.pdf}
%%\includegraphics[width=5cm]{Kappa100GeV.pdf}
%%\caption{The ratio of $\sigma_{1/p_\mathrm{T}}$ to the average of GLD, GLDPrime, and GLD4LDC models,
%%   as a function of the track angle, for muons of energy 1, 10, and 100 GeV.}
%%\label{fig:mreso_ene}
%%\end{figure}

\subsection{Impact Parameter Resolution}

The impact parameter resolution, $\sigma_{r\phi}$, of the tracking system is
an important input to the heavy flavour tagging capability of the detector.
The most important detector considerations are the vertex detector
design (point resolution and material budget) and the magnetic field
which, as discussed in Section~\ref{sec:optimization-background} affects 
the minimum distance of the first layer of the vertex detector from the
interaction region, $R_\mathrm{min}$. 
Figure~\ref{fig:ipreso}a shows 
$\sigma_{r\phi}$ as a function 
of $p_{\mathrm{T}}$ for the GDC-based
detector models. The GLD4LDC model has the best resolution, 
because the higher $B$-field 
allows the innermost layer of the vertex detector to be closer to the 
interaction point (IP). However the differences between the detector
models considered, Figure~\ref{fig:ipreso}b, are relatively small $\lesssim 5-10$\,\%. 

\begin{figure}
\begin{center}
\includegraphics[width=7.cm]{d0res.pdf}
\includegraphics[width=7.cm]{d0ResRatio.pdf}
\includegraphics[width=7.cm]{rphi.pdf}
\includegraphics[width=7.cm]{rphiPt.pdf}
\caption[Impact parameter resolution.]{(a) $\sigma_{r\phi}$ as a function of $p_{\mathrm{T}}$ 
for GLD, GLDPrime, and GLD4LDC, and (b) the ratio of $\sigma_{r\phi}$ to the average of the three detector models.
c) $\sigma_{r\phi}$ as a function of the track angle at the 
track energy of 1 GeV for GLD, GLDPrime, and GLD4LDC. d) 
the impact parameter resolution as a function of $p_{\mathrm{T}}$ 
for GLDPrime and LDCPrime. Also
shown is the nominal ILC goal for impact parameter resolution.
\label{fig:ipreso}}
\end{center}
\end{figure}


Figure \ref{fig:ipreso}c shows the $\sigma_{r\phi}$ resolution for 1\,GeV muons
for the GLD-based detector models, plotted as a function of the track angle.
Whilst the higher magnetic fields are favoured, the differences 
between the detector models are $\lesssim 15\,\%$. For higher energy tracks,
where the effect of multiple Coulomb scattering is negligible, the differences 
between the models are even smaller. 
Although the variations in magnetic field and the corresponding inner radii 
of the vertex detector lead to relatively small differences in impact parameter
resolution, different detector layouts have a more significant impact. Figure 
\ref{fig:ipreso}d compares the 
impact parameter resolution for the GLDPrime and 
LDCPrime detector models. The GLDPrime detector 
assumes a vertex detector consisting of
six layers arranged in three closely spaced doublets 
(see Section~\ref{ild:vertex}),
whereas the LDCPrime model assumes five equally spaced layers. 
The three double layer layout results in a significantly better
impact parameter resolution for high momentum tracks 
because it gives two, rather than one, high precision 
measurements close to the IP.  


\subsection{Conclusions}

For the range of $B$ and $R$ considered here,
the differences in momentum resolution are $\lesssim10$\,\%,
with higher $B$-field preferred for low $p_{\mathrm{T}}$ tracks 
and a larger $R$ preferred for high $p_{\mathrm{T}}$ tracks.
The impact parameter resolution, $\sigma_{r\phi}$, is better for
models with higher $B$ as the first layer of the vertex detector
can be placed closer to the IP. However, the differences in impact
parameter resolution obtained with a 3\,T and 4\,T magnetic field are small, 
at most 15\,\% for low momentum tracks and $\lesssim5\,\%$ for tracks above
2\,GeV. It can be concluded that for the range of $B$ and $R$ spanned
by the LDC and GLD detector concepts, the differences in 
impact parameter and momentum resolution are relatively small.
It is also concluded that the tracking resolutions depend much 
more strongly on the subdetector technologies and tracking system
layout than on the global parameters ($B$ and $R$) of the detector.


